BEHAVIOR Vision Suite: Customizable Dataset Generation via Simulation

The systematic evaluation and understanding of computer vision models under varying conditions require large amounts of data with comprehensive and customized labels, which real-world vision datasets rarely satisfy. While current synthetic data generators offer a promising alternative, particularly for embodied AI tasks, they often fall short for computer vision tasks due to low asset and rendering quality, limited diversity, and unrealistic physical properties. We introduce the BEHAVIOR Vision Suite (BVS), a set of tools and assets to generate fully customized synthetic data for systematic evaluation of computer vision models, based on the newly developed embodied AI benchmark, BEHAVIOR-1K. BVS supports a large number of adjustable parameters at the scene level (e.g., lighting, object placement), the object level (e.g., joint configuration, attributes such as "filled" and "folded"), and the camera level (e.g., field of view, focal length). Researchers can arbitrarily vary these parameters during data generation to perform controlled experiments. We showcase three example application scenarios: systematically evaluating the robustness of models across different continuous axes of domain shift, evaluating scene understanding models on the same set of images, and training and evaluating simulation-to-real transfer for a novel vision task: unary and binary state prediction. Project website: https://behavior-vision-suite.github.io/

==> 999-text-grave.tex <==

% BV-Suite consists of two main parts: BV-Asset and a Customized-Dataset-Generator (CDG).
% The BV-Suite is composed of two primary components: BV-Asset and the Customized-Dataset-Generator (CDG). BV-Asset features a library of over 8,000 photorealistic objects and more than 1,000 diverse simulated scenes. The CDG leverages this extensive asset pool, offering complete customization capabilities for crafting datasets specifically designed to enhance the training and assessment of perception models. The datasets generated can be finely tuned with custom annotations, object and scene arrangements, and specific graphics distributions: 
% Our BV-Suite produces datasets with detailed annotations aimed at holistic scene understanding for robotic perception, supporting evaluations across multiple tasks. The CDG generates over 10,000 RGB-D video trajectories within complex indoor environments, enriched by more than 15 annotation types, which are critical for both comprehensive scene analysis and the development of innovative open-vocabulary understanding models.
% Additionally, the CDG tailors object and scene configurations for spatial relationship analysis, employing a strategic cycle from real-world to simulation and back, generating synthetic data and digital twins. Models trained on this data demonstrate impressive skill in interpreting real-world scenarios through sim2real transfer. The BV-Suite also adapts graphic distributions to challenge and assess parametric models, effectively simulating domain shifts to test model robustness. Overall, our efforts highlight the transformative impact of photorealistic simulations in advancing visual perception technologies.

%% Raw version
% Real-world vision datasets, constrained by their static nature and lack of controllability, often falter in vision tasks that need customized and flexible dataset. Especially for those tasks that interested in special object composition, environment condition (lighting, occlusion) and comprehensive labels. Recently, using simulation data shows a promising solution for emboded AI task, while still challenge for vision task, mainly due to the relatively low asset quality, limited asset size and diversity and lack of physically plausible property, which show large domain gap with real data.
% Addressing the pressing challenges faced in real-world and simulation data, we propose BEHAVIOR Vision Suite (BV-Suite) for customized vision dataset generation with Realistic 3D asset and simulation. 
% BV-Suite consists of two main parts: BV-Asset and a Customized-Dataset-Generator (CDG).
% BV-Asset consists over 8,000 meticulously crafted, photo-realistic objects and more than 1,000 simulated scene instances. Anchored by its full controllability, the innovative CDG showcases its potential in curating datasets tailored to elevate perception model training and evaluation. 
% We show the generated dataset could have customized annotations, object \& scene composition, and graphics distribution: we generate dataset with comprehensive annotations for holistic scene understanding in robotic perception—a discipline demanding simultaneous evaluations across diverse tasks. CDG crafts a dataset enriched with 10k+ RGB-D video trajectories in intricate indoor settings, augmented by 15+ types of annotations. This not only propels holistic scene model evaluations but also underpins the formulation of a pioneering open-vocabulary holistic scene understanding model. 
% CDG also customize object \& scene composition to generate dataset for the spatial relationship understanding task, BDG employs a judicious real-to-simulation-to-real strategy, autonomously birthing synthetic data, and subsequently, a digital twin. Models nurtured on this synthetic data have manifested commendable adeptness in discerning real-world dynamics, thanks to the sim2real transfer mechanism. Additionally, BDG offers customized graphics distribution during dataset generation ideal for rigorous parametric model evaluations. It adeptly simulates domain shifts, setting a challenging arena to discern the strengths and pinpoint the Achilles' heel of varied models against our benchmark. Collectively, our work underscores the immense potential of photo-realistic simulation and assets in revolutionizing visual perception.


% Real-world datasets, constrained by their static nature and lack of controllability, often falter in scene understanding, label precision, and task-specific adaptability. This rigidity limits customization essential for key real-world tasks. We propose BEHAVIOR Asset as a solution, which consists over 7,000 meticulously crafted, photo-realistic objects and more than 2,000 simulated scenes. Anchored by its full controllability, the innovative BEHAVIOR-Dataset-Generator (BDG) showcases its potential in curating datasets tailored to elevate perception model training and evaluation. For holistic scene understanding in robotic perception—a discipline demanding simultaneous evaluations across diverse tasks—BDG crafts a dataset enriched with 10k+ RGB-D video trajectories in intricate indoor settings, augmented by 15+ types of annotations. This not only propels holistic scene model evaluations but also underpins the formulation of a pioneering open-vocabulary holistic scene understanding model. Transitioning to the spatial relationship understanding task, BDG employs a judicious real-to-simulation-to-real strategy, autonomously birthing synthetic data, and subsequently, a digital twin. Models nurtured on this synthetic data have manifested commendable adeptness in discerning real-world dynamics, thanks to the sim2real transfer mechanism. Additionally, in a testament to its adaptability, BDG offers customized dataset generation ideal for rigorous parametric model evaluations. It adeptly simulates domain shifts, setting a challenging arena to discern the strengths and pinpoint the Achilles' heel of varied models against our benchmark. Collectively, our work underscores the immense potential of photo-realistic simulation and assets in revolutionizing visual perception.


% Real-world datasets, constrained by their static nature and lack of controllability, often falter in scene understanding, label precision, and task-specific adaptability. This rigidity limits customization essential for key real-world tasks. The BEHAVIOR Asset emerges as a solution, bridging these gaps with flexibility, adequacy and precision. This robust collection boasts over 7,000 meticulously crafted, photo-realistic objects and more than 2,000 simulated scenes. Anchored by its full controllability, the innovative BEHAVIOR-Dataset-Generator (BDG) showcases its potential in curating datasets tailored to elevate perception model training and evaluation. For holistic scene understanding in robotic perception—a discipline demanding simultaneous evaluations across diverse tasks—BDG crafts a dataset enriched with 10k+ RGB-D video trajectories in intricate indoor settings, augmented by 15+ types of annotations. This not only propels holistic scene model evaluations but also underpins the formulation of a pioneering open-vocabulary holistic scene understanding model. Transitioning to the spatial relationship understanding task, BDG employs a judicious real-to-simulation-to-real strategy, autonomously birthing synthetic data, and subsequently, a digital twin. Models nurtured on this synthetic data have manifested commendable adeptness in discerning real-world dynamics, thanks to the sim2real transfer mechanism. Additionally, in a testament to its adaptability, BDG offers customized dataset generation ideal for rigorous parametric model evaluations. It adeptly simulates domain shifts, setting a challenging arena to discern the strengths and pinpoint the Achilles' heel of varied models against our benchmark. Collectively, our work underscores the immense potential of photo-realistic simulation and assets in revolutionizing visual perception.

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Teaser image to show the }
%    \label{fig:teaser}
% \end{figure}

  % % motovation
  % Real-world datasets frequently encounter challenges in areas such as holistic scene understanding, complex label acquisition, and customization for specific application needs. Addressing these challenges, we introduce the BEHAVIOR Asset—a collection enriched with high-quality, photo-realistic assets and realistic simulations. This asset consists of an impressive 7,000+ objects and 2,000+ scenes. With its full controllability, we demonstrate how it can be adeptly utilized to create holistic, tailored, and cost-efficient datasets that significantly enhance perception model evaluation and training. We frame the dataset generation approach as BEHAVIOR-Dataset-Generator (BDG)
  % % Our solution
  % % 1 holistic scene understanding
  % We first show how BDG generate comprehensive annotated dataset for holistic scene understanding in robotics perception, which requires model evaluations across multiple tasks in identical environments. Specifically, we create a holistic seene understanding evaluation dataset which contains 10k+ RGB-D video trajectories on complex indoor scene with 15+ types of annotations. We show how the generated benchmark dataset help holistic scene understanding model evaluation and we propose a new open-vocabulary holistic scene understanding baseline model. 
  % % 2 Cost-Effective Data Acquisition
  % Then, we show BDG can help cost-effective dataset generation for spatial relationship understanding task. We follow a real-to-simulati on-to-real approach, autonomously generating synthetic data and creating a digital twin. Our results demonstrate that models trained on this synthetic data exhibit strong performance in understanding real-world scenes through sim2real transfer.
  % % 3 parametrc model evaluation
  % BDG also provide customized dataset generation for Parametric Model evaluation, which designed to simulate domain shift to aggressively probe the boundaries and identify failure cases of different models using our benchmark. 




  % % motovation [version before Sept. 14]
  %  3D Scene Graph (3DSG) Reconstruction, which integrates object-level, scene-level, and relationship details, is pivotal for perception in embodied AI and robotics. However, the field lacks a large-scale 3DSG reconstruction evaluation benchmark, mainly due to the demanding nature of extensive annotations. Interactive, physically-accurate virtual simulations can bridge this gap. Addressing this need, we introduce BEHAVIOR4Perception, a comprehensive 3D Scene Graph benchmark encompassing both synthetic and real scene data. It showcases more than 7,000 objects across 2,000 scenes, enriched by detailed annotations across over 15 modalities.
  %  % Benchmark
  %  BEHAVIOR4Perception facilitates a thorough assessment on the demanding task of 3DSG reconstruction. The 3DSG amalgamates object-level data, such as 2D masks, 3D meshes, 6D poses, and unary predicates, with scene-level details including depth, layout, point cloud, and binary spatial relationships. Significantly, these graphs also encapsulate dynamic annotations, illuminating robot or camera trajectories.
  %  % Baseline model to solve the benchmark
  %  We introduce the first Open-vocabulary 3D Scene Reconstruction model (O-3DSG). This pioneer solution leverages open-vocabulary vision-language models to derive 3DSG from video data. 
  %  % Usage of the Benchmark 
  %  BEHAVIOR4Perception provide a new evaluation metric for 3DSG reconstruction models. 
  %  Alongside this, we introduce the Parametric Model evaluation (PME) pipeline, designed to simulate domain shift to aggressively probe the boundaries and identify failure cases of different models using our benchmark. 
  %  To tackle the sim2real challenge, BEHAVIOR4Perception operates as a Real2Sim2real engine, autonomously generating synthetic data and creating a digital twin. Our results demonstrate that models trained on this synthetic data exhibit strong performance in understanding real-world scenes through sim2real transfer.
  % % motovation
  %  How can physically-plausible, interactive virtual simulations help advancing the real-world physical scene understanding and embodied AI? To address this, we introduce BEHAVIOR-Asset, a large-scale photo-realistic 3D Geometric Scene Graph benchmark dataset encompassing over 7,000 objects and 50 realistic scenes with comprehensive, over 20 modalities annotations. 
  %  % BEHAVIOR-Asset evaluate 3GSG task
  %  BEHAVIOR-Asset empowers a comprehensive evaluation on challenging 3D Geometric Scene Graph (3GSG) reconstruction task, which requires object-level, scene-level, and dynamic-level ground truths, a central goal for visual perception models equipped on embodied agents. The 3GSG effectively combines object-level annotations, such as 2D masks, 3D meshes, 6D poses, and unary attributes with scene-level annotations like depth, layout, point cloud, and binary spatial relationships. Moreover, these graphs capture dynamic annotations detailing robot or camera trajectories.
  %  % Modeling, evaluation
  %  We present a Open-vocabulary 3D Geometric Scene Understanding Engine (O-3GSE), the first baseline solution that utilizes open-vocabulary foundational vision-language models to reconstruct 3GSG from video inputs. Alongside this, we introduce the Parametric Extreme Model evaluation (PEE) pipeline, designed to systematically assess different models using our benchmark. To bridge the sim2real gap, we introduce a Sim2real engine designed to automatically generate synthetic data, enhancing the model's capability in real-world scene understanding.


  % % motovation
  %  How could physically-plausible, interactive virtual simulation help advancing the real-world physical scene understanding and embodied AI? To explore this problem, we propose BEHAVIOR-Asset, a large-scale photo-realistic 3D Geometric Scene Graph benchmark dataset encompassing over 7,000 objects and 50 realistic scenes with comprehensive, over 20 modalities annotations. 
  %  % BEHAVIOR-Asset evaluate 3GSG task
  %  BEHAVIOR-Asset empowers a systematic evaluation on challenging 3D Geometric Scene Graph (3GSG) reconstruction task, which requires object-level, scene-level, and dynamic-level ground truths, a ultimate goal of visual perception model equipped on embodied agents. Specifically, 3GSG seamlessly merge object-level annotations, including 2D masks, 3D meshes, 6D poses, unary attributes with scene-level annotations, notably depth, lay out, point cloud, and binary spatial relationships. Moreover, these graphs capture dynamic annotations detailing robot or camera trajectories.
  %  % Modeling, evaluation
  %  We propose the first baseline solution, Open-vocabulary 3D Geometric Scene Understanding Engine (O-3GSE), that harnesses open-vocabulary foundational vision-language models to reconstruct 3GSG from video inputs. We propose a Parametric Extreme Model evaluation (PEE) pipeline to systemically evaluate different models with our benchmark. We also present a Sim2real engine that automatically generate synthetic data to improve the performance on real spatial relationship understanding. 
   
   
   
   
   % In the pursuit of advancing the fields of physical scene understanding, augmented reality, and robotics, we introduce the BEHAVIOR-Asset: a large-scale Dynamic Geometric Scene Graph benchmark dataset. Encompassing 7,000+ objects and 50+ richly annotated scenes, BEHAVIOR-Asset provides an unprecedented depth of data on object-level, scene-level, and dynamic ground truths. 
   % To process input videos of indoor scene explorations, we introduce Dynamic Geometric Scene Graphs. These intricate structures combine a myriad of annotations, ranging from object semantics, spatial relationships, 2D/3D representations, and 6D poses, to scene-focused annotations like camera poses and depth, and even dynamic annotations detailing robot or camera trajectories. 
   % To navigate this rich dataset, we present a novel baseline solution, using foundational vision models to reconstruct Dynamic Geometric Scene Graphs from video inputs. Our approach is distinguished by its focus on understanding spatial relationships, predicting binary relationships between objects with precision. To gauge the efficacy of our approach, we rigorously assess current state-of-the-art methods for tasks like 6D pose and depth estimation. Preliminary trials utilizing our baseline solution in robotics tasks have yielded promising results, underscoring the potential benefits of our contributions to the research community.


% Enhanced Perception Dataset Generation:

% Holistic Scene Understanding:
% Our approach directly responds to the compelling need for evaluations that span across multiple tasks within identical environments. With the BEHAVIOR Asset, we present a dataset that not only meets, but surpasses current standards. It offers comprehensive annotations, encapsulating over 2,000 scenes, 7,000 objects, and an impressive 10,000+ RGB-D video trajectories, all embellished with more than 15 types of annotations. Such extensive coverage ensures an all-encompassing environment comprehension, vital for cutting-edge robotic perception tasks.

% Cost-Effective Data Acquisition for Complex Tasks:
% The intricate nature of acquiring specific labels, such as understanding spatial relationships, often comes with prohibitive costs. We tackle this challenge head-on, deploying a novel real-to-simulation-to-real paradigm. This methodology streamlines data acquisition for these multifaceted tasks, ensuring both feasibility and cost-effectiveness.

% Customization for Specific Needs:
% Moving away from the limitations that bind generic datasets, our approach offers unparalleled customization capabilities. Whether the requirement is for scenarios with extreme low lighting or specific occlusions, our assets stand ready. Beyond mere customization, the BEHAVIOR Asset introduces a robust mechanism for parametric evaluation, empowering researchers to accurately assess model performance under these tailor-made distributions.

% In essence, our contributions coalesce to form a paradigm shift in visual perception dataset generation. By fusing high-quality assets with a photo-realistic simulator, we not only bridge existing gaps but chart a promising trajectory for future advancements in the field. The BEHAVIOR Asset and its dataset generation capabilities embody a monumental stride in ensuring that visual perception systems are both comprehensive and tailored to specific needs, all the while ensuring cost efficiency.



%% Motivation

% Why 3DSG important and shortcomings of current benchmarks
% 3D Scene Graph (3DSG) reconstruction stands as a pivotal technique for scene understanding, embodied AI, and robotics, given its ability to integrate object-level, scene-level, and relationship information. Yet, the domain faces a salient challenge: the lack of a large-scale benchmark for 3DSG reconstruction evaluation. This limitation arises chiefly from the demanding need for exhaustive annotations. Current methods, as referenced in [1,2], are primarily evaluated on: (1) Real 3D scene datasets of smaller scales, often hindered by incomplete annotations (for instance, Gisbon’s tiny split).
% (2) Simulated datasets, such as uHumans, that span only 3 scenes and miss out on photo realistic accuracy.
% Notably, several existing 3D scene understanding benchmarks, like ScanNet and ARKitScenes, fall short of facilitating 3DSG reconstruction evaluation. This is predominantly because of their insufficient annotations. While simulators have the potential to generate more annotations, they often compromise on the photorealistic quality of scenes.

% Why use simulator
% Simulations offer a compelling solution when crafting benchmarks for several reasons. Firstly, they are inherently controllable and can auto-generate vast quantities of 3D scene graph data. This means we can effortlessly access rich annotations—ranging from 2D and 3D bounding boxes, segmentation, depth, to scene point clouds and more. Notably, the cost of obtaining such varied annotations is practically zero.
% Moreover, the adaptability of simulations ensures a vast diversity in data. This includes variations in room layouts, lighting conditions, camera configurations, and levels of occlusion—all without added effort or cost. And while the authenticity of simulated data is often under scrutiny, if crafted with photorealistic precision, it can become invaluable for real-world tasks.
% The data generated through simulation can be seamlessly leveraged for both evaluation and training, thus providing a comprehensive toolkit for advancements in the field

% BEHAVIOR4Perception Benchmark
% In an effort to address these challenges, we present the BEHAVIOR4Perception benchmark. This comprehensive tool is designed as a large-scale 3DSG reconstruction benchmark dataset, covering both photorealistic synthetic and real scenes. It contains an extensive collection of over 2000 scenes, 7000+ 3D objects, and 10,000+ RGB-D video trajectories. Additionally, it features more than 15 types of annotations, which span scene-level, object-level, and dynamic-level labels, all meticulously structured as 3DSG. 

% 3DSG reconstruction task demands precision at multiple granularities: object-level, scene-level, and dynamic-level ground truths. Meeting these stringent requirements is paramount for the efficacy of visual perception models, especially those tailored for embodied agents that interact closely with their environments. The 3DSG, a cornerstone of our dataset, is adept at seamlessly integrating a myriad of annotations. On the object-level, it brings together vital details such as 2D semantic masks, 3D meshes, accurate 6D poses, and unary attributes, such as open/close, burned, cooked, sliced, frozen, that define singular properties of entities. Simultaneously, it dives deeper into the scene, capturing annotations that detail the depth, layout, and point cloud information, providing a holistic spatial understanding. This is further enriched by binary spatial relationships that depict how different objects relate within the scene, such as above, under, inside. Beyond static relationships, BEHAVIOR-Asset excels in documenting the dynamics of a setting. The graphs incorporate annotations that chronicle the movement and trajectories, be it of robots navigating the environment or cameras capturing the scene, providing a temporal dimension to the spatial understanding.

% Our Baseline to solve the task
% The Open-vocabulary 3D Scene Graph Reconstruction model (O-3DSG) is introduced as the first baseline solution that leverages open-vocabulary foundational vision-language models to reconstruct 3DSG from video inputs. 

% % a systemetic evaluation method
% In addition to the O-3GSE, we present the Parametric Model Evaluation (PME) pipeline. This evaluation framework is meticulously crafted to appraise a range of models using BEHAVIOR4Perception as the standard benchmark. Employing PME entails dynamically altering the test set distribution to aggressively probe the boundaries and identify failure cases of each model. Consequently, this detailed scrutiny provides an in-depth analysis of each model's performance metrics, guaranteeing a comprehensive evaluation.
% For those real perception task that hard to obtain labels, we propose Real2Sim2Real pipeline. Empowered by our BEHAVIOR dataset generator, This pipeline is engineered to autonomously produce synthetic data that mirrors real-world dynamics, with the primary objective of enhancing model accuracy during transitions from simulated to real-world contexts. As a case in point, utilizing spatial understanding, we demonstrate that by employing our Real2Sim2Real engine, it becomes feasible to train a spatial prediction model exclusively on synthetic data, yet achieve commendable performance in actual real-world settings.

% Here are the main contributions: 
% (1) We propose BEHAVIOR4Perception, a benchmark for 3D Scene Graph (3DSG) reconstruction, amassing an extensive collection of data from over 2,000 synthetic and real scenes, encompassing more than 7,000 objects and 10,000+ RGB-D video trajectories, each with over 15 diverse annotation types. (2) We introduce a pioneering Open-vocabulary 3DSG reconstruction baseline model, capable of processing video input to render a comprehensive scene understanding represented as 3DSG, augmented by advanced vision foundation models. (3) Our benchmark serves multiple utilities, ranging from assessing both comprehensive and partial solution 3DSG reconstruction models to facilitating rigorous out-of-distribution parametric testing, targeting diverse domain shifts. A Real2Sim2Real pipeline is also featured, autonomously generating synthetic data and creating a digital twin. Our results demonstrate that models trained on this synthetic data exhibit strong performance in understanding real-world scenes through sim2real transfer.

%%%%%%% Back up
% % Motivation
% Understanding physical scenes in a 3D environment is foundational for embodied AI. Yet, as the field progresses, there is a heightened need for robust, scalable, and comprehensive benchmarking datasets to evaluate these simulations. Acquiring labeled data from the real world is both time-intensive and costly.

% Physically plausible virtual environments offer a potential solution for generating evaluation benchmarks suited for complex robotics tasks. Several platforms, such as BEHAVIOR, iGibson, and ProcThor, have emerged in response. However, the extent to which physically-plausible, interactive virtual simulations can enhance real-world physical scene understanding remains an area of active investigation.
% There are two primary challenges persist:
% \textbf{Photo-realism in Virtual Environments}: The visual quality of virtual simulations is pivotal for perception tasks. Currently, many assets fall short of achieving photo-realism. This gap exacerbates the 'sim2real' evaluation challenges and can potentially hinder model generalization.
% \textbf{Comprehensive Annotations across Modalities}: A benchmarking dataset should ideally encompass annotations covering a broad spectrum of modalities to be truly effective. This ensures the holistic evaluation of algorithms and systems under varying conditions and tasks. \textbf{Real-to-Sim-to-Real Solution}: : The process of transitioning from real-world requirements to creating their digital counterparts in a simulator, and then utilizing that simulated data to enhance real-world scene understanding, presents a significant challenge. Specifically, the methodology for systematically closing the loop between real and simulated environments remains ambiguous. Establishing this loop is pivotal, as it would enable a seamless integration of virtual simulations with real-world applications, optimizing the performance of embodied AI systems.

% % Our method
% To address this pressing need, we present BEHAVIOR-Asset, which offering stands as a landmark in benchmark datasets, boasting a large-scale, photo-realistic, 3D Geometric Scene Graph structure. Its vastness is underscored by the inclusion of over 7,000 intricately detailed objects, spread across 50 meticulously crafted, lifelike scenes. But BEHAVIOR-Asset is not just about size; it's about depth and breadth. Each element within the dataset is accompanied by comprehensive annotations, spanning a wide range of more than 20 diverse modalities. This ensures that every facet of the objects and scenes is captured, offering researchers an unparalleled resource for in-depth analyses and applications.

% % BEHAVIOR-Asset evaluate 3GSG task
% BEHAVIOR-Asset stands as a pivotal tool in advancing the field of 3D Geometric Scene Graph (3GSG) reconstruction, a domain known for its intricate challenges. This reconstruction task demands precision at multiple granularities: object-level, scene-level, and dynamic-level ground truths. Meeting these stringent requirements is paramount for the efficacy of visual perception models, especially those tailored for embodied agents that interact closely with their environments. The 3GSG, a cornerstone of our dataset, is adept at seamlessly integrating a myriad of annotations. On the object-level, it brings together vital details such as 2D semantic masks, 3D meshes, accurate 6D poses, and unary attributes, such as open/close, burned, cooked, sliced, frozen, that define singular properties of entities. Simultaneously, it dives deeper into the scene, capturing annotations that detail the depth, layout, and point cloud information, providing a holistic spatial understanding. This is further enriched by binary spatial relationships that depict how different objects relate within the scene, such as above, under, inside. Beyond static relationships, BEHAVIOR-Asset excels in documenting the dynamics of a setting. The graphs incorporate annotations that chronicle the movement and trajectories, be it of robots navigating the environment or cameras capturing the scene, providing a temporal dimension to the spatial understanding.

% % Our Baseline
% The Open-vocabulary 3D Geometric Scene Understanding Engine (O-3GSE) is introduced as the first baseline solution that leverages open-vocabulary foundational vision-language models to reconstruct 3D Geometric Scene Graphs (3GSG) from video inputs. The engine's primary function is to transform real-world scenes into a structured format that can be processed computationally.

% % a systemetic evaluation method
% In addition to the O-3GSE, we present the Parametric Extreme Model evaluation (PEE) pipeline. This evaluation framework is meticulously crafted to appraise a range of models using BEHAVIOR-Asset as the standard benchmark. Employing PEE entails dynamically altering the test set distribution to aggressively probe the boundaries and identify failure cases of each model. Consequently, this detailed scrutiny provides an in-depth analysis of each model's performance metrics, guaranteeing a comprehensive evaluation.

% Recognizing the prevalent 'sim2real' gap, wherein models trained on simulated data often underperform in real-world scenarios, we introduce the BEHAVIOR Sim2real engine. This system is engineered to autonomously produce synthetic data that mirrors real-world dynamics, with the primary objective of enhancing model accuracy during transitions from simulated to real-world contexts. As a case in point, utilizing spatial understanding, we demonstrate that by employing our Sim2real engine, it becomes feasible to train a spatial prediction model exclusively on synthetic data, yet achieve commendable performance in actual real-world settings.

% Here are the main contributions: 
% (1) We developed BEHAVIOR-Asset, a comprehensive 3D Geometric Scene Graph benchmark dataset, characterized by its photo-realism, physically-plausible, interactive, and encompassing over 7,000 objects across 50 lifelike scenes with exhaustive annotations spanning 20+ modalities for applications in physical scene understanding and embodied AI. 
% (2) For input videos depicting indoor scene explorations, we've crafted 3D Geometric Scene Graph that merge object-level, scene-level, and dynamic annotations, capturing details ranging from 6D poses to camera trajectories.
% (3) We propose the first baseline solution, Open-vocabulary 3D Geometric Scene Understanding Engine (O-3GSE), utilizing open-vocabulary vision-language models to convert video inputs of real-world scenes into computationally structured 3D Geometric Scene Graphs (3GSG).
% (4))Additionally, we present the Sim2real engine to autonomously generate synthetic data, mitigating challenges associated with transitioning models from simulated to real-world environments.


% Our solution
% We present our pioneering contributions: the meticulously crafted BEHAVIOR assets and a state-of-the-art realistic simulation that's both physically plausible and grounded in functionality.
% BEHAVIOR Assets: A Quantum Leap in Data Quality:
% Our first significant contribution is the high quality BEHAVIOR assets. This expansive collection encompasses over 2,000 intricately designed scenes and a staggering 7,000 3D objects (including articulation objects). Such assets don't just serve as a mere repository; they lay the foundation for creating datasets that resonate with real-world scenarios, ensuring a seamless transition from theory to practical implementation.
% Realistic Simulation: The Bedrock of Authenticity:
% Complementing our assets is the realistic simulation, anchored in physical plausibility. Beyond mere visual mimicry, our simulator incorporates genuine physical grounding functionalities, bridging the chasm between conventional simulated environments and real-world dynamics.
% BEHAVIOR-Dataset-Generator (BDG): Turning Possibilities into Realities:
% Armed with the BEHAVIOR assets and the realistic simulator, we introduce the BEHAVIOR-Dataset-Generator (BDG), a testament to what's achievable when high-quality resources meet innovative design:



% Backup

% Physical scene understanding in 3D world is important and the foundation of embodied AI. However, as the domain rapidly evolves, so does the demand for robust, scalable, and comprehensive benchmarking datasets tailored to evaluate of these simulations. Real world labelled data is time and money consuming.
% Physical plausible Virtual environment provide a solution for creating evaluation benchmark for complex robotics. For instance, BEHAVIOR, igibson, ProcThor. However, it is unclear how can physically-plausible, interactive virtual simulations help advancing the real-world physical scene understanding task. 
% There are few challenges: (1) Photo-realistic requirement of the virtual environment. Appearance quality is important for perception task, most of the current asses are far from photo-realistic, which enlarge the sim2real evaluation gap and make limit the model generalization.
% (2) fulfilled annotations of all modalities.


% BEHAVIOR Asset Details: Here, we delve into the intricacies of BEHAVIOR assets, emphasizing its comprehensive collection of over 7,000 objects and 50 scenes. These high-caliber, photorealistic components serve as the paper's cornerstone.

% Dataset Generation and Utility: This section elucidates how BEHAVIOR supports the formulation of datasets for varying purposes:

% A broad perspective is given on the benchmark task of Geometric Spatial Scene Graph (GSSG) reconstruction, discussing its motivation, evaluation metrics, and the expansive dataset.
% Additionally, for more niche domain tasks, we concentrate on Unary and binary predicate predictions. We spotlight the Real 2 Sim 2 Real methodology, beginning with genuine needs, transitioning to a digital replica in BEHAVIOR, and finally to sim2real transfer. We accentuate the invaluable traits of synthetic data, notably its endless quantity and full controllability.
% Evaluation: In this concluding section, we unveil the premier fully automatic Geometric Spatial Perception Engine (GSPE) crafted to fashion a GSSG from visual-inertial data. Our modular solution amalgamates cutting-edge techniques for diverse subtasks such as 2D/3D reconstruction. Through multi-task learning, these subtasks reinforce one another. Our experimental assessments, while not necessarily achieving top scores, provide profound insights. Additionally, the exploration of spatial relationships and a proposed evaluation pipeline for foundational vision models are discussed.




% Main contributions:

% 1 We build BEHAVIOR-Asset, which is a large-scale Dynamic Geometric Scene Graph benchmark dataset, that contains 5,000 objects, and 50 scenes annotated with rich physical and semantic properties. This benchmark features object-level, scene-level, and dynamic ground truths, crucial for advanced applications in physical scene understanding, augmented reality, and robotics.

% 2 In response to an input video of an indoor scene exploration, we devise Dynamic Geometric Scene Graphs. These Graphs integrate object-level annotations, including semantic labels, 2D masks, 3D meshes, 6D poses, spatial relationships, and unary predicates. Additionally, they cover scene-level annotations, such as camera pose, room layout, and depth. Finally, they include dynamic annotations that capture robot or camera trajectories.

% 3 We put forth a baseline solution that employs foundational vision models to reconstruct a Dynamic Geometric Scene Graph from an input video. Our approach uniquely incorporates a spatial relationship understanding method that predicts the binary relationships between objects. Furthermore, we conduct an in-depth evaluation of the state-of-the-art methods for specific tasks, such as 6D pose estimation and depth estimation.

% 4 We utilize the baseline solution to conduct trials on various robotics tasks, demonstrating encouraging outcomes that suggest the potential applicability and effectiveness of our proposed methods and resources.
